End-to-End O-RAN Security Architecture, Threat Surface, Coverage, and the Case of the Open Fronthaul

O-RAN establishes an advanced radio access network (RAN) architecture that supports inter-operable, multi-vendor, and artificial intelligence (AI) controlled wireless access networks. The unique components, interfaces, and technologies of O-RAN differentiate it from the 3GPP RAN. Because O-RAN supports 3GPP protocols, currently 4G and 5G, while offering additional network interfaces and controllers, it has a larger attack surface. The O-RAN security requirements, vulnerabilities, threats, and countermeasures must be carefully assessed for it to become a platform for 5G Advanced and future 6G wireless. This article presents the ongoing standardization activities of the O-RAN Alliance for modeling the potential threats to the network and to the open fronthaul interface, in particular. We identify end-to-end security threats and discuss those on the open fronthaul in more detail. We then provide recommendations for countermeasures to tackle the identified security risks and encourage industry to establish standards and best practices for safe and secure implementations of the open fronthaul interface.

==> include/ORAN_threats_SecurityTable.tex <==
\begin{table*}
%\renewcommand{\arraystretch}{1.3}
% \setlength{\arrayrulewidth}{0.15mm}
% \setlength{\doublerulesep}{0.12mm}
\centering
\caption{O-RAN threats and coverage security principles.}
\footnotesize
\label{tab:Table1}
\centering
{\begin{tabular}{|p{0.8cm}|p{1.0cm}|p{6.8cm}|p{3.7cm}|p{3.1cm}|}
\hline
\multicolumn{2}{|c|}{\textbf{O-RAN Component}}  &\textbf{Threat } &  \textbf{Affected Components} &  \textbf{Security Principles} 
\\ \hline
%\multirow{3}{*}
{Front-haul}
& 
Fronthaul 
&
\textcolor{black}{- {An attacker penetrates O-DU and beyond through O-RU or the Fronthaul interface.}} 
\newline - {Unauthorized access to Open Front Haul Ethernet L1 physical layer interface(s).}
& 
rApps, xApps, O-RU, O-DU, O-CU, Near-RT RIC, Non-RT RIC.
&
Mutual authentication, access control, cryptographic, key management, PKI, trusted Communication, and security assurance. 
\\
\cline{2-4}
&
M-Plane 
&
\textcolor{black}{- {An attacker attempts to intercept the Fronthaul (MITM) over M Plane.}} 
& 
rApps, xApps, O-RU, O-DU, O-CU, Near-RT RIC, Non-RT RIC.
&
\\

\cline{2-4}
& %\rule{0pt}{4ex}   
{S-Plane} 
& 
\textcolor{black}{- {DoS attack against a Master clock. }} 
\newline - {Impersonation of a Master clock (Spoofing) within a PTP network with a fake ANNOUNCE message}.
\newline - {A Rogue PTP Instance wanting to be a Grand Master}.
\newline - {Selective interception and removal of PTP timing packets}.
\newline - {Packet delay manipulation attack}.
&
O-DU, O-RU.
&
\\
\cline{2-4}

& 
%SDR 
C-Plane  
& 
\textcolor{black}{- {Spoofing of DL C-plane messages.}}
\textcolor{black}{- {Spoofing of UL C-plane messages.}}
& 
O-DU, O-RU.
&
\\
\cline{2-4}

& 
%SDR 
U-Plane  
& 
\textcolor{black}{- {An attacker attempts to intercept the Fronthaul (MITM) over U Plane.}} 
& 
O-DU, O-RU.
&
\\
\hline
%\multirow{3}{*}
{Near-RT RIC} 
& 
\rule{0pt}{3ex} Near-RT RIC 
& 
\textcolor{black}{- Malicious Apps can exploit UE identification, track UE location and change UE priority.}
&
Near-RT RIC, UE, xApps.
&
SB, OPNS, ASSU, PRV, SLC, ISO, CLD
\\

%\makecell{1 W or 15 W PA (ground node) \\1 W PA (aerial node)\\ LNA on both receive chains}&
\cline{2-5}
& \rule{0pt}{4ex}    {xAPPs}  
& 
\textcolor{black}{- An attacker exploits xApps vulnerabilities and misconfiguration.} 
\newline \textcolor{black}{- Conflicting xApps unintentionally or maliciously impact O-RAN system functions to degrade performance or trigger a DoS.}
\newline - An attacker compromises xApp isolation. 
&
O-CU, Near-RT RIC, xApps
&
AUTH, ACC, CRYPTO, SB, UPDT, RECO, ASSU, SLC, ISO, CLD    
\\
\hline
%\multirow{2}{*}
{Non-RT RIC} 
& 
Non-RT RIC 
& 
\textcolor{black}{- {An attacker penetrates the non-RT RIC to cause a denial of service or degrade the performance.} }
\newline \textcolor{black}{- UE sniffing in the Non-RT RIC.}
&
Non-RT RIC, rApps, UE.
&
AUTH, ACC, CRYPTO, ASSU, PRV, SLC, SB, OPNS, CLD
\\

\cline{2-5}

& 
rAPPs  & 
\textcolor{black}{- {An attacker exploits rApps vulnerabilities and misconfiguration.} } 
\newline \textcolor{black}{- An attacker bypasses authentication and authorization.}
\newline \textcolor{black}{- An attacker compromises rApp isolation.}
\newline \textcolor{black}{- Conflicting rApps unintentionally or maliciously impact O-RAN system functions to degrade performance or trigger a DoS.}
&
rApps, UE, Non-RT RIC, Near-RT RIC, xApps.
&
AUTH, ACC, CRYPTO, SB, UPDT, RECO, ASSU, SLC, ISO, CLD  
\\
\hline
%\multirow{2}{*}
\multicolumn{2}{|c|}{\textbf{SMO}} 
&  
\textcolor{black}{- {An attacker can exploit the improper/missing authentication weakness on SMO functions.} } 
\newline \textcolor{black}{- An attacker can exploit the improper/missing authorization weakness on SMO functions.}
\newline \textcolor{black}{- Overload DoS attacks at SMO.}
&
SMO components.
&
AUTH, ACC, UPDT, RECO, ASSUS, SLC
\\
\hline
%\multirow{2}{*}
\multicolumn{2}{|c|}{\textbf{O-CLOUD}} 
&
{
\textcolor{black}{- An attacker compromises VNF/CNF images and embedded secrets. }}
\newline \textcolor{black}{- An attacker exploits weak orchestrator configuration, access control and isolation.}
\newline \textcolor{black}{- Misuse of a VM/CN to attack other VM/CN, hypervisor/container engine, other hosts (memory, network, storage), etc.}
\newline \textcolor{black}{- Spoofing and eavesdropping on network traffic.}
\newline \textcolor{black}{- An attacker compromises auxiliary/supporting network and security services.}
& 
O-Cloud components.
&
AUTH, ACC, CRYPTO, SS, SB, UPDT, RECO, OPNS, ASSU, SLC, ISO, CLD
\\
\hline
\multicolumn{2}{|c|}{\textbf{ML/AI}} 
&
{
\textcolor{black}{- Poisoning the ML training data (Data poisoning attacks). }}
\newline \textcolor{black}{- An attacker exploits weak orchestrator configuration, access control and isolation.}
\newline \textcolor{black}{- Altering a machine learning model (System manipulation and compromise of ML data confidentiality and privacy).}
\newline \textcolor{black}{- Spoofing and eavesdropping on network traffic.}
\newline \textcolor{black}{- Transfer learning attack.}
& 
Near-RT RIC, Non-RT RIC, xAPPs, rApps.
&
AUTH, ACC, CRYPTO, SB, UPDT, RECO, ASSU,  SLC, ISO, CLD
\\
\hline
\end{tabular}
\vspace{-3 mm}
}
\end{table*}

==> include/projects.tex <==
%Projects related to UAS Communications
%- Development, deployment and testing projects: AERPAW, Ericsson trials, Qualcomm trials, ... Adding research projects is fine as long as they are not about stochastic geometry or purely theoretical/simulation based. I would focus on experimental R&D. 
While UAS communications research and standardization are still in their early stages, important %global 
R\&D %research
projects and testbeds are being established. These %projects 
are necessary %mainly built 
to study the performance requirements of UAVs and evaluate the technology and protocol solutions to support the various use cases in real-life scenarios. Repeatable experimental results obtained in controlled, yet production-like environments, will in return accelerate advancing communications %promote the efforts to %finalize
%advance the 
standards. 
\begin{itemize}

\item \textbf{AERPAW [https://aerpaw.org]}: The Aerial Experimentation and Research Platform for Advanced Wireless (AERPAW) is being built in the US since 2019 under the Platforms for Advanced Wireless Research (PAWR) program. 
%COSMOS, lead by Rutgers University, NYU, and Columbia University, enables research on advanced wireless and networking technologies, such as mm-wave, 5G, Edge and Cloud computing. 
%POWDER/RENEW, lead by University of Utah in collaboration with Rice University, focuses on research on spectrum sharing and massive MIMO. 
AERPAW is a unique large-scale testbed enabling experimentation with advanced wireless technology and systems for UAVs. 
%mobile radio nodes s, lead by NC State in collaboration with Mississippi State University, WRC and RENCI, will allow advanced wireless research with unmanned aerial vehicles (UAVs).
%All these platforms are or will soon be open to global researchers and can be remotely accessed for running research experiments. 
The goal of AERPAW is to support global 5G and Beyond 5G wireless research on connected 3D mobility, spectrum agility and security, and 3D network topology, among others. 
AERPAW will therefore offer access to commercial-grade 5G technology and networks as well as to software radios that can be programmed to implement many different waveforms and protocols. These radios will be deployed on several fixed nodes and be available as payloads for UAVs. 
An emulator and sandbox will enable development and pre-testbed deployment of new radios, networks and experiments.% \cite{aerpaw-GC19}. 
%if, for example, strong jamming or other attacks are of interest and are not possible on the over-the-air testbed. (Vuk)
\vspace{+1 mm}
\item \textbf{5G!Drones [https://5gdrones.eu]:} In June 2019, a three-year European project named 5G!Drones %~\cite{5GDrones}
has kicked offed. Academia has joined forces with industry and includes network operators and research centers for testing UAV use cases over 5G networks. The use cases that are considered in this project includes: UAV traffic management, public safety, and situational awareness. The trails aim to validate the %5G 
ability to support aerial services and provide feedback that can be used to improve the performance of 5G systems for the selected use cases. 5G!Drones is part of Phase 3 of the 5G %Infrastructure 
Public Private Partnership (5GPPP) projects funded by the European Commission.
\vspace{+1 mm}
\item \textbf{5G-DIVE [https://5g-dive.eu]:} In October 2019, a collaboration %teams consist 
of %various %verticals,
vendors, service providers, network
operators, small or medium-sized enterprises (SMEs), academic and research centers from %both
the EU and Taiwan established the 5G-DIVE project. %~\cite{5GDive}. 
5G-DIVE plans to perform field and real-life tests of different 5G technologies to ensure technical merits and business value proposition are fulfilled, before advancing those technologies to higher levels. The %5G-DIVE project's 
trails mainly focus on %the 
Industry 4.0 use cases, such as digital twin app and real time video analysis for zero defect manufacturing. The second trails focus on %cases are the
autonomous drone scouting %use cases
involving drone fleet
navigation and intelligent processing of images captured by the
drones. %~\cite{5GDIVE_paper}.
5G-DIVE is funded by the European Union through the H2020 Program. % for two years.
\end{itemize}
%\hl{Skyward and Verizon:} In April 2017, Verizon started working closely with the Skyward team~\cite{skyward} to enhance Skyward drone solutions and promote its operation with emphasis on management and safety of drone operations. Through this cooperation, the Skyward drones %operations 
%will enjoy advanced wireless connectivity that can provide more flexibility to the aerial operations at low cost. Currently, Skyward's solutions are ready for the Airborne LTE Operations (ALO) enabled by Verizon's networks %technology 
%and they plan %working 
%to test the 5G solution soon. %The 
%5G %solution 
%will provide %a great
%advantages for %the
%aerial operations, such as remote aircraft deployments, simultaneous control of multiple drones, better performance awareness and analysis %analytics 
%using artificial intelligence and enabling fully autonomous drone operations.%~\cite{verizon}.       
%
%\hl{Valqari smart mailbox delivery startup:?}
%
